EditCLIP: Representation Learning for Image Editing

We introduce EditCLIP, a novel representation-learning approach for image editing. Our method learns a unified representation of edits by jointly encoding an input image and its edited counterpart, effectively capturing their transformation. To evaluate its effectiveness, we employ EditCLIP to solve two tasks: exemplar-based image editing and automated edit evaluation. In exemplar-based image editing, we replace text-based instructions in InstructPix2Pix with EditCLIP embeddings computed from a reference exemplar image pair. Experiments demonstrate that our approach outperforms state-of-the-art methods while being more efficient and versatile. For automated evaluation, EditCLIP assesses image edits by measuring the similarity between the EditCLIP embedding of a given image pair and either a textual editing instruction or the EditCLIP embedding of another reference image pair. Experiments show that EditCLIP aligns more closely with human judgments than existing CLIP-based metrics, providing a reliable measure of edit quality and structural preservation.

==> sec/0_abstract.tex <==
\begin{abstract}
We introduce \abbrv, a novel representation-learning approach for image editing.  
Our method learns a unified representation of edits by jointly encoding an input image and its edited counterpart, effectively capturing their transformation.  
To evaluate its effectiveness, we employ \abbrv to solve two tasks: exemplar-based image editing and automated edit evaluation.  
In exemplar-based image editing, we replace text-based instructions in InstructPix2Pix \cite{brooks2023instructpix2pix} with \abbrv embeddings computed from a reference exemplar image pair.  
Experiments demonstrate that our approach outperforms state-of-the-art methods while being more efficient and versatile.  
For automated evaluation, \abbrv assesses image edits by measuring the similarity between the \abbrv embedding of a given image pair and either a textual editing instruction or the \abbrv embedding of another reference image pair.  
Experiments show that \abbrv aligns more closely with human judgments than existing CLIP-based metrics, providing a reliable measure of edit quality and structural preservation.
\vspace{-5mm}

% Unlike existing CLIP-based metrics, which struggle to capture fine-grained details and excessive deviations from the original image, \abbrv effectively addresses these limitations, offering a scalable, automated alternative to human evaluations. 
\end{abstract}

==> tables/bench.tex <==
\begin{table*}[!t]
\caption{Statistics of pairs after creating examplar pairs using \citet{kawar2023imagic} benchmark.}
\label{tab:corr}
\centering
%%% BEGIN COPY PASTE BELOW FROM df.to_latex(), only changed column titles below after

\begin{tabular}{lr}
\toprule
Edit name & Num of pairs \\
\midrule
boy2girl & 50 \\
midnight & 50 \\
seapainting & 50 \\
sketchstyle & 60 \\
summer & 55 \\
wallpaper & 55 \\
charcoal & 60 \\
glasses & 50 \\
painting & 60 \\
paintingsnow & 50 \\
pencilsketch & 50 \\
purple & 32 \\
snow & 50 \\
watercolor & 40 \\
4dboy & 50 \\
apple & 50 \\
cake & 50 \\
cloud\_kitty & 50 \\
dog2cat & 55 \\
juice & 50 \\
lava & 50 \\
rain & 50 \\
read\_books & 50 \\
smile & 50 \\
traffic\_lights & 60 \\
\bottomrule
total & 1277 \\
\bottomrule
\end{tabular}
%%% END COPY PASTE BELOW FROM df.to_latex()
\end{table*}

==> tables/correlation.tex <==

\begin{table*}[!t]
\caption{Statistical analysis on GenAI-Bench\citet{li2024genaibenchevaluatingimprovingcompositional}.}
\label{tab:corr}
\centering
%%% BEGIN COPY PASTE BELOW FROM df.to_latex(), only changed column titles below after
\begin{tabular}{lrrrrrr}
\toprule
Metric & Condorcet Count & Win Ratio & Mean Winning Score & Pearson & Spearman & Kendall \\
\midrule
editclip & 354 & 0.704 & 0.216 & 0.442 & 0.460 & 0.376 \\
editclip\_desc & 331 & 0.658 & 0.257 & 0.325 & 0.339 & 0.277 \\
editclip\_dir & 351 & 0.698 & 0.108 & 0.456 & 0.465 & 0.380 \\
editclip\_dir\_images & 241 & 0.479 & 0.411 & -0.018 & -0.032 & -0.026 \\
lpips & 327 & 0.650 & 0.220 & 0.393 & 0.390 & 0.319 \\
clip & 344 & 0.684 & 0.277 & 0.419 & 0.423 & 0.346 \\
clip\_dir & 386 & 0.767 & 0.180 & 0.549 & 0.576 & 0.471 \\
clip\_image & 311 & 0.618 & 0.878 & 0.272 & 0.285 & 0.233 \\
l1 & 306 & 0.608 & 0.045 & 0.179 & 0.222 & 0.182 \\
l2 & 304 & 0.604 & 0.005 & -0.011 & 0.145 & 0.118 \\
ssim & 332 & 0.660 & 0.724 & 0.309 & 0.330 & 0.270 \\
psnr & 304 & 0.604 & 20.802 & 0.174 & 0.187 & 0.153 \\
dino & 334 & 0.664 & 0.866 & 0.372 & 0.386 & 0.315 \\
\bottomrule
\end{tabular}
%%% END COPY PASTE BELOW FROM df.to_latex()

\end{table*}
